A Multi-Agent Security Testbed for the Analysis of Attacks and Defenses in Collaborative Sensor Fusion

The performance and safety of autonomous vehicles (AVs) deteriorates under adverse environments and adversarial actors. The investment in multi-sensor, multi-agent (MSMA) AVs is meant to promote improved efficiency of travel and mitigate safety risks. Unfortunately, minimal investment has been made to develop security-aware MSMA sensor fusion pipelines leaving them vulnerable to adversaries. To advance security analysis of AVs, we develop the Multi-Agent Security Testbed, MAST, in the Robot Operating System (ROS2). Our framework is scalable for general AV scenarios and is integrated with recent multi-agent datasets. We construct the first bridge between AVstack and ROS and develop automated AV pipeline builds to enable rapid AV prototyping. We tackle the challenge of deploying variable numbers of agent/adversary nodes at launch-time with dynamic topic remapping. Using this testbed, we motivate the need for security-aware AV architectures by exposing the vulnerability of centralized multi-agent fusion pipelines to (un)coordinated adversary models in case studies and Monte Carlo analysis.

==> algorithms/algorithm_attacks.tex <==
\begin{algorithm}
\caption{Uncoordinated target selection for adversary $i$.}\label{alg:uncoord-selection}
\begin{algorithmic}
\Require Number of FN/FP: $k_{FN},\, k_{FP}$, Max range for FP: $\rho_{\text{max}}$
\Ensure targets
\State $D \gets$ \texttt{receive\_detections($\text{agent}_i$)}
    \State targets[FN] $\gets$ \texttt{random\_choice}($D$, $k_{FN}$)
    \State targets[FP] $\gets$ \texttt{random\_state}($\rho_{\text{max}}$, $k_{FP}$)
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{Coordinated target selection at coordinator.}\label{alg:coord-selection}
\begin{algorithmic}
\Require Number of FN/FP: $k_{FN},\, k_{FP}$, Max range for FP: $\rho_{\text{max}}$
\Ensure targets
\State $\mathcal{D} \gets$ \{\texttt{receive\_detections($\text{agent}_j$)} $\forall \ j$\}
\State $\mathcal{P} \gets$ \{\texttt{receive\_pose($\text{agent}_j$)} $\forall \ j$\}
\State $\mathcal{D} \gets$ \{\texttt{align\_frames($D_j,\, P_j$)} $\forall \ j$\}
\State $C \gets$ \texttt{clustering($\mathcal{D}$)}
\State targets[FN] $\gets$ \texttt{random\_choice}($C$, $k_{FN}$)
\State targets[FP] $\gets$ \texttt{random\_state}($\rho_{\text{max}}$, $k_{FP}$)

\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{Attack execution.}\label{alg:attack-exec}
\begin{algorithmic}
\Require Number of FN/FP: $k_{FN},\, k_{FP}$, Max range for FP: $\rho_{\text{max}}$
\State $\text{initialized} \gets \text{False}$
\While{True}
\State $D \gets$ \texttt{receive\_detections()}
\If{\texttt{not} initialized}
    \State targets $\gets$ \texttt{select\_targets($D$)}
    \State initialized $\gets$ True
\EndIf
\State idx\_remove $\gets$ \texttt{assignment}($D$, targets[FN])
\State targets[FN] $\gets$ $D$[idx\_remove]
\State targets[FP] $\gets$ \texttt{propagate}(targets[FP])
\State $D \gets$ $D$[\texttt{not} idx\_remove] + targets[FP]
\State \texttt{send\_detections}($D$)
\EndWhile
\end{algorithmic}
\end{algorithm}


==> figures/ros-framework-nodes.tex <==
\begin{figure*}
    \centering
    \includesvg[width=\linewidth]{diagrams/rosgraph.svg}
    \caption{ROS nodes from a 3-agent configuration generated from \texttt{rqt\_graph} ROS plugin. Simulation from the \avstack\ multi-agent dataset~\cite{hallyburton2023datasets} provides event-driven execution. Two infrastructure agents and one mobile agent (``ego'') provide tracked information to the command center namespace. All tracks are pushed to the visualizer for real-time feedback. ROS framework automatically scales to the number of agents in the simulation.}
    \label{fig:ros-framework}
\end{figure*}

==> figures/safety-critical-pipeline.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{example-image-b}
    \caption{Safety-critical functionality driven by algorithms based on local information to mitigate impact of external adversaries.}
    \label{fig:safety-critical-pipeline}
\end{figure}
